Can LLM Judges Catch Unsafe Clinical Actions? A Fault-Injection Study

As clinical AI agents begin to interact with electronic health records (EHRs), large language models (LLMs) are increasingly used to evaluate their actions. But how reliably can these judges recognize clinically dangerous mistakes, especially when an agent appears to have completed its task successfully? We investigate this question using MedAgentBench by introducing controlled clinical errors into verified agent trajectories. The experiments include 416 faulty trajectories, eight error categories, and six open-weight LLM judges. By comparing each faulty trajectory with its correct counterpart, we measure whether judges genuinely recognize errors rather than simply flagging more actions as unsafe. The findings show that access to clinical evidence significantly improves judge reliability. When shown only the final answer, judges cannot distinguish errors that leave it unchanged, while flagging 56% of correct trajectories. With full trajectory information, the ability to distinguish unsafe actions from correct ones reaches a score of 0.75, and providing actual EHR responses improves discrimination by 0.39. Surprisingly, including the agent's reasoning does not improve overall performance and reduces detection of incorrectly reported clinical values by 0.18, which remain the hardest errors to detect. MedGemma performed worse than the general-purpose model and was the only judge to miss potentially dangerous medication overdoses. We also find that the benchmark's original grader accepts all 38 trajectories with an intentionally skipped laboratory check, while combining LLM judges with a rule-based checker informed by the full EHR record detects 97% of injected faults.

==> results/tab_agents_rows.tex <==
% agent & episodes & grader pass % & passes flagged by checker % & clean candidates
gpt-oss 120B & 630 & 48 & 0.7 & 301 \\
Qwen3 32B & 630 & 45 & 2.5 & 277 \\


==> results/tab_hyp_rows.tex <==
% id & contrast & estimate [95% CI] & Holm-adjusted p
H1 & V1: $\Delta$ (answer same) $\approx 0$ & $-$0.01 [$-$0.03, 0.00] & $<$0.001 \\
H2 & V3: $\Delta$(F1--F3) $-$ $\Delta$(F5, F7) & 0.22 [0.14, 0.29] & 1.000 \\
H3$^{e}$ & V3: $\Delta$(S3) $-$ $\Delta$(S0--S2) & 0.16 [0.07, 0.24] & 0.993 \\
H4 & F6: $\Delta$(V3n) $-$ $\Delta$(V2) & 0.64 [0.57, 0.71] & $<$0.001 \\
H6 & V3: $\Delta$(MedGemma) $-$ $\Delta$(Gemma 3) & $-$0.08 [$-$0.14, $-$0.02] & $<$0.001 \\
H7$^{e}$ & V3: sens.(own) $-$ sens.(other family) & $-$0.10 [$-$0.15, $-$0.05] & $<$0.001 \\


==> results/tab_judges_rows.tex <==
% judge & Delta V1-I1 & Delta V3-I2 [95% CI] & sensitivity % & false alarm % & critical miss % [95% CI] & paired AUROC & ECE (all V3-I2)
Qwen3 8B$^{r}$ & $-$0.04 & 0.67 [0.58, 0.76] & 87 & 13 & 0 [0, 0] & 0.46 & 0.26 \\
Qwen3 32B$^{r}$ & 0.04 & 0.81 [0.76, 0.87] & 89 & 5 & 0 [0, 0] & 0.66 & 0.17 \\
gpt-oss 20B$^{r}$ & $-$0.01 & 0.69 [0.63, 0.75] & 71 & 1 & 0 [0, 0] & 0.62 & 0.30 \\
gpt-oss 120B$^{r}$ & $-$0.04 & 0.77 [0.67, 0.86] & 96 & 14 & 0 [0, 0] & 0.63 & 0.28 \\
Gemma 3 27B & 0.02 & 0.81 [0.76, 0.86] & 85 & 3 & 0 [0, 0] & 0.52 & 0.28 \\
MedGemma 27B$^{m}$ & $-$0.02 & 0.73 [0.68, 0.79] & 78 & 3 & 33 [8, 67] & 0.55 & 0.31 \\


==> results/tab_judges_side_rows.tex <==
% as tab_judges_rows.tex, but paired AUROC and ECE use the stated score read on the side of the verdict (see confidence_check.csv)
Qwen3 8B$^{r}$ & $-$0.04 & 0.67 [0.58, 0.76] & 87 & 13 & 0 [0, 0] & 0.86 & 0.10 \\
Qwen3 32B$^{r}$ & 0.04 & 0.81 [0.76, 0.87] & 89 & 5 & 0 [0, 0] & 0.93 & 0.07 \\
gpt-oss 20B$^{r}$ & $-$0.01 & 0.69 [0.63, 0.75] & 71 & 1 & 0 [0, 0] & 0.81 & 0.19 \\
gpt-oss 120B$^{r}$ & $-$0.04 & 0.77 [0.67, 0.86] & 96 & 14 & 0 [0, 0] & 0.93 & 0.03 \\
Gemma 3 27B & 0.02 & 0.81 [0.76, 0.86] & 85 & 3 & 0 [0, 0] & 0.94 & 0.09 \\
MedGemma 27B$^{m}$ & $-$0.02 & 0.73 [0.68, 0.79] & 78 & 3 & 33 [8, 67] & 0.89 & 0.15 \\


==> results/tab_severe_rows.tex <==
% condition & S3 faults rated by every judge & S3 missed % [95% CI] & S2+S3 missed % [95% CI] & S3 missed by all judges & S3 missed by a majority
V1--I1 & 12 & 11 [3, 21] & 32 [26, 39] & 0 & 0 \\
V1--I2 & 12 & 21 [12, 31] & 37 [32, 42] & 0 & 0 \\
V2--I1 & 12 & 0 [0, 0] & 13 [10, 17] & 0 & 0 \\
V2--I2 & 12 & 0 [0, 0] & 16 [13, 20] & 0 & 0 \\
V3n--I2 & 11 & 3 [0, 8] & 9 [7, 12] & 0 & 0 \\
V3--I1 & 12 & 8 [4, 13] & 10 [7, 12] & 0 & 0 \\
V3--I2 & 12 & 6 [1, 11] & 14 [11, 18] & 0 & 0 \\
V3--I3 & 12 & 3 [0, 7] & 12 [9, 15] & 0 & 0 \\


==> results/tab_stack_rows.tex <==
% fault & mutants & detected by the grader % & by the step checker % & by the judges (mean of judges, V3-I2) % & by a majority of judges % & by none of the three %
F1 Wrong patient & 60 & 100 & 100 & 98 & 100 & 0 \\
F2 Dose magnitude & 18 & 100 & 100 & 93 & 100 & 0 \\
F3 Unit swap & 60 & 100 & 30 & 99 & 100 & 0 \\
F4 Ignored observation & 60 & 100 & 100 & 78 & 85 & 0 \\
F5 Skipped precondition & 38 & 0 & 100 & 95 & 95 & 0 \\
F6 Hallucinated observation & 60 & 100 & 70 & 49 & 35 & 0 \\
F7 False completion & 60 & 100 & 100 & 80 & 90 & 0 \\
F8 Wrong code & 60 & 100 & 0 & 95 & 100 & 0 \\
\midrule
All faults & 416 & 91 & 71 & 84 & 87 & 0 \\


==> results/tab_view_rows.tex <==
% condition & Delta answer-unchanged [95% CI] & Delta answer-changed [95% CI] & critical miss % [95% CI] & false alarm % [95% CI]
V1--I1 & $-$0.01 [$-$0.03, 0.00] & 0.01 [$-$0.05, 0.06] & 11 [3, 21] & 56 [51, 61] \\
V1--I2 & $-$0.01 [$-$0.03, 0.01] & 0.00 [$-$0.06, 0.05] & 21 [12, 31] & 54 [49, 59] \\
V2--I1 & 0.49 [0.41, 0.57] & 0.10 [0.05, 0.15] & 0 [0, 0] & 44 [39, 50] \\
V2--I2 & 0.46 [0.38, 0.54] & 0.16 [0.11, 0.21] & 0 [0, 0] & 39 [34, 44] \\
V3n--I2 & 0.81 [0.75, 0.86] & 0.68 [0.62, 0.73] & 3 [0, 8] & 7 [5, 9] \\
V3--I1 & 0.80 [0.74, 0.86] & 0.69 [0.64, 0.74] & 8 [4, 13] & 8 [6, 11] \\
V3--I2 & 0.81 [0.75, 0.86] & 0.59 [0.53, 0.64] & 6 [1, 11] & 6 [4, 9] \\
V3--I3 & 0.83 [0.78, 0.88] & 0.65 [0.60, 0.70] & 3 [0, 7] & 6 [4, 8] \\

